Assessing Test-time Variability for Interactive 3D Medical Image Segmentation with Diverse Point Prompts

Interactive segmentation model leverages prompts from users to produce robust segmentation. This advancement is facilitated by prompt engineering, where interactive prompts serve as strong priors during test-time. However, this is an inherently subjective and hard-to-reproduce process. The variability in user expertise and inherently ambiguous boundaries in medical images can lead to inconsistent prompt selections, potentially affecting segmentation accuracy. This issue has not yet been extensively explored for medical imaging. In this paper, we assess the test-time variability for interactive medical image segmentation with diverse point prompts. For a given target region, the point is classified into three sub-regions: boundary, margin, and center. Our goal is to identify a straightforward and efficient approach for optimal prompt selection during test-time based on three considerations: (1) benefits of additional prompts, (2) effects of prompt placement, and (3) strategies for optimal prompt selection. We conduct extensive experiments on the public Medical Segmentation Decathlon dataset for challenging colon tumor segmentation task. We suggest an optimal strategy for prompt selection during test-time, supported by comprehensive results. The code is publicly available at https://github.com/MedICL-VU/variability

==> text/text_old/_0-abstract_old.tex <==
% Recently, to tackle the label availability problem in medical
% image segmentation, parameter-efficient model adaptation
% methods have leveraged knowledge from pretrained image
% foundation models, such as the Segment Anything Model
% (SAM), to optimize and achieve robust performance. This
% advancement is facilitated by prompt engineering, where in-
% teractive prompts serve as strong priors during test-time to
% deliver the reliable segmentations. However, the ambigu-
% ous boundaries often present in medical images can lead to
% variability in prompt selection, which may yield different
% results, especially for challenging tumor segmentation. Ad-
% ditionally, to date, no prior research has been conducted on
% this issue within medical imaging contexts. In this paper, we
% assess the test-time variability of a pretrained network that
% has been adapted from a foundational model with prompt
% engineering for medical image segmentation. Specifically,
% point prompts are used during validation. Since labeling
% medical images is an expensive and time-consuming process,
% we aim to investigate the clear-cut and effort-free improve-
% ments at inference: (1) the necessary number of prompts;
% (2) the optimal locations for prompt selection to achieve
% optimized results; and (3) the impact of different prompts
% on segmentation outcomes. Our experiments are conducted
% using the public Medical Segmentation Decathlon (MSD)
% dataset for colon tumor segmentation. We suggest an optimal
% solution for prompt selection during test-time, supported by
% comprehensive results

==> text/text_old/_1-introduction_old.tex <==


Medical image segmentation is essential for simplifying images into task-specific representations, facilitating easier analysis. 
To date, deep learning methods have demonstrated superior performance in various segmentation tasks \cite{liu2023medical}. However, the generalizability and performance of such methods may be limited by the amount of available training data, especially for the labeled data \cite{wang2023ssl2}. Obtaining labeled data in medical imaging is challenging due to the costly imaging acquisition and the time-consuming process of human delineation.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{image/variability.pdf}   
\caption{The illustrations of a interactive segmentation model (top), which takes an image and a point prompt as inputs, while the bottom illustrates its test-time variability with different prompts provided by expert. Best viewed in color.}
\label{variability}
\end{figure}

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{image/point_selection.pdf}   
\caption{The details of various point prompt selection strategies are depicted through 2D illustrations. From left to right: (a) ground truth, highlighting the entire tumor area; (b) random selection throughout the entire tumor; (c) placement selection confined to a specific region; (d) strategy selection C, where the initial point (denoted by a triangle) is considered a fixed reference with cumulative points (circles) varying between iterations; and (e) strategy selection I, characterized by initial points that shift position while cumulative points remain stationary. Different colors represent different iterations (or runs).
}
\label{point_sampling}
\end{figure*}

To improve generalizability of segmentation model, interactive segmentation methods that integrate user knowledge and application requirements are adopted for more robust segmentation performance \cite{wang2018interactive} (see Fig.~\ref{variability} (top)). To further tackle the data and label availability issue in medical imaging, it is desired to utilize knowledge from the natural images domain, wherein large public datasets are more readily accessible \cite{matsoukas2022makes}. Recent studies have leveraged insights from pretrained natural image foundation models, such as the Segment Anything Model (SAM) \cite{kirillov2023segment}, which is trained on massive datasets, to facilitate robust medical image segmentation through parameter-efficient transfer learning techniques \cite{ma2023segment,wu2023medical,gong20233dsam,li2023promise,deng2023sam,zhang2023input,zhang2023segment}. The interactive pattern of these methods that use diverse visual prompts, such as point and box, can achieve superior performance due to the strong prior provided by the given prompt during test-time inference. Moreover, point prompts are preferable in practice, which requires less effort to provide, especially for 3D medical images.

In practice, medical image segmentation often relies on sparse in-house datasets due to the lack of large public training set. Moreover, transferring data between imaging sites is challenging with privacy concerns. Alternatively, test-time techniques are widely used for a given pretrained model \cite{wang2019aleatoric,li2022self,zhang2023input} to achieve superior segmentations. For interactive segmentation models, different users may have varying levels of expertise, leading to inconsistencies in the prompt choice and segmentation process \cite{schmidt2023probabilistic,cheng2023sam} at test-time, an illustration is shown in Fig.~\ref{variability} (bottom). Towards this end, we aim to investigate the optimal strategy for point prompt selection for pretrained interactive segmentation models at test-time inference. To the best of our knowledge, no existing work has explicitly addressed prompt selection in the medical field.




In this paper, we firstly validate the test-time variability on prompt selection of prompt-driven 3D medical image segmentation model to bring an insight for future study (Fig.~\ref{variability}). Specifically, we use the ProMISe \cite{li2023promise} as the backbone which leverages the pretrained weights from SAM \cite{kirillov2023segment}. It takes image and point prompts as inputs to produce segmentation. We evaluate the variability with different prompts at inference to understand how such interactive models respond to varying point prompts. To provide a pragmatic solution, our investigation focuses on three questions (Fig.~\ref{point_sampling}): (1) whether additional prompts are beneficial, (2) the influence of prompt placement, and (3) the strategy for selecting prompts to optimize outcomes. We conduct our evaluation on colon tumor segmentation from the public Medical Segmentation Decathlon dataset \cite{antonelli2022medical}, which is characterized by irregular shapes and ambiguous boundaries. The findings from comprehensive result suggest that a clear-cut and effort-free test-time prompt selection, leading to improved segmentation results over random prompt selection.



















